Type Ia Supernovae are Excellent Standard Candles in the Near-Infrared

We analyze a set of 89 Type Ia supernovae (SN Ia) that have both optical and near-infrared (NIR) photometry to derive distances and construct low redshift ($z < 0.04$) Hubble diagrams. We construct mean light curve (LC) templates using a hierarchical Bayesian model. We explore both Gaussian process (GP) and template methods for fitting the LCs and estimating distances, while including peculiar velocity and photometric uncertainties. For the 56 SN Ia with both optical and NIR observations near maximum light, the GP method yields a NIR-only Hubble-diagram with a RMS of $0.117 \pm 0.014$ mag when referenced to the NIR maxima. For each NIR band, a comparable GP method RMS is obtained when referencing to NIR-max or B-max. Using NIR LC templates referenced to B-max yields a larger RMS value of $0.138 \pm 0.014$ mag. Fitting the corresponding optical data using standard LC fitters that use LC shape and color corrections yields larger RMS values of $0.179 \pm 0.018$ mag with SALT2 and $0.174 \pm 0.021$ mag with SNooPy. Applying our GP method to subsets of SN Ia NIR LCs at NIR maximum light, even without corrections for LC shape, color, or host-galaxy dust reddening, provides smaller RMS in the inferred distances, at the $\sim 2.3 - 4.1\sigma$ level, than standard optical methods that do correct for those effects. Our ongoing RAISIN program on the Hubble Space Telescope will exploit this promising infrared approach to limit systematic errors when measuring the expansion history of the universe to constrain dark energy.

==> tables/carrick_Flow_corrections_snnames2.tex <==
SN2009Y & 220.59938 & -17.24678 & NGC 5728 & 2793 $\pm$ 8 & 3019 $\pm$ 9 & 2827 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009aa & 170.92617 & -22.27069 & ESO 570-G20 & 8187 $\pm$ 14 & 8543 $\pm$ 15 & 8597 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009ab & 64.15162 & 2.76417 & UGC 2998 & 3349 $\pm$ 6 & 3260 $\pm$ 6 & 3090 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009ad & 75.88908 & 6.65992 & UGC 3236 & 8514 $\pm$ 1 & 8496 $\pm$ 1 & 8602 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009ag & 107.92004 & -26.68508 & ESO 492-2 & 2590 $\pm$ 2 & 2774 $\pm$ 2 & 3056 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009al & 162.84196 & 8.57853 & NGC 3425 & 6627 $\pm$ 24 & 6982 $\pm$ 25 & 7007 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009an & 185.69750 & 65.85111 & NGC 4332 & 2764 $\pm$ 2 & 2867 $\pm$ 2 & 3207 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009bv & 196.83542 & 35.78444 & MCG +06-29-039 & 10966 $\pm$ 5 & 11201 $\pm$ 5 & 11539 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009cz & 138.75008 & 29.73531 & NGC 2789 & 6344 $\pm$ 3 & 6601 $\pm$ 3 & 6548 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009kk & 57.43458 & -3.26444 & 2MFGC 03182 & 3855 $\pm$ 45 & 3729 $\pm$ 44 & 3653 $\pm$ 150 & NED;C15 & Flow \\ 
SN2009kq & 129.06292 & 28.06722 & MCG +05-21-001 & 3507 $\pm$ 6 & 3739 $\pm$ 6 & 3766 $\pm$ 150 & NED;C15 & Flow \\ 
SN2010ai & 194.85000 & 27.99639 & SDSS J125925.04+275948.2 (Coma) & 5507 $\pm$ 37 & 7166 $\pm$ 54 & 7298 $\pm$ 150 & NED;P14 & Cluster \\ 
SN2010dw & 230.66792 & -5.92111 & 2MASX J15224062-0555214 & 11428 $\pm$ 45 & 11600 $\pm$ 46 & 11759 $\pm$ 150 & NED;C15 & Flow \\ 
SN2010iw & 131.31250 & 27.82278 & UGC 4570 & 6458 $\pm$ 2 & 6698 $\pm$ 2 & 6833 $\pm$ 150 & NED;C15 & Flow \\ 
SN2010kg & 70.03500 & 7.35000 & NGC 1633 & 4986 $\pm$ 2 & 4931 $\pm$ 2 & 5128 $\pm$ 150 & NED;C15 & Flow \\ 
SN2011B & 133.95208 & 78.21750 & NGC 2655 & 1400 $\pm$ 1 & 1419 $\pm$ 1 & 1670 $\pm$ 150 & NED;C15 & Flow \\ 
SN2011ao & 178.46250 & 33.36278 & IC 2973 & 3210 $\pm$ 1 & 3487 $\pm$ 1 & 3592 $\pm$ 150 & NED;C15 & Flow \\ 
SN2011by & 178.94000 & 55.32611 & NGC 3972 & 852 $\pm$ 1 & 1521 $\pm$ 61 & 1796 $\pm$ 150 & NED;R16 & Cepheid \\ 
SN2011df & 291.89000 & 54.38639 & NGC 6801 & 4361 $\pm$ 6 & 4205 $\pm$ 6 & 4500 $\pm$ 150 & NED;C15 & Flow \\ 
SNf20080514-002 & 202.30625 & 11.26889 & UGC 8472 & 6577 $\pm$ 3 & 6866 $\pm$ 3 & 6480 $\pm$ 150 & NED;C15 & Flow \\ 


==> tables/table1header.tex <==
\tiny
\begin{tabular}{lrr c cc rcc} 
\hline \hline
\multicolumn{1}{l}{SN name$^{a}$}        & \multicolumn{1}{c}{$RA$ (deg)}            & \multicolumn{1}{c}{$DEC$ (deg)}         & \multicolumn{1}{c}{Host Galaxy}     & \multicolumn{1}{c}{$\vhel$}        & \multicolumn{1}{c}{$\vcmb$}  & \multicolumn{1}{c}{$\vcmbf$} & 
\multicolumn{1}{c}{Ref(s).$^{g}$} &
\multicolumn{1}{c}{Code$^{h}$}  \\ 
\multicolumn{1}{l}{} &
\multicolumn{1}{r}{$\alpha(2000)^{b}$} & \multicolumn{1}{r}{$\delta(2000)^{b}$}  & \multicolumn{1}{c}{(or cluster)$^{c}$} & \multicolumn{1}{c}{(km s$^{-1}$)$^{d}$}        & \multicolumn{1}{c}{(km s$^{-1}$)$^{e}$}   & \multicolumn{1}{c}{(km s$^{-1}$)$^{f}$} & \multicolumn{1}{c}{} & 
\multicolumn{1}{c}{} \\ 
